Quantum thermodynamic devices: from theoretical proposals to experimental reality

Thermodynamics originated in the need to understand novel technologies developed by the Industrial Revolution. However, over the centuries the description of engines, refrigerators, thermal accelerators, and heaters has become so abstract that a direct application of the universal statements to real-life devices is everything but straight forward. The recent, rapid development of quantum thermodynamics has taken a similar trajectory, and, e.g., "quantum engines" have become a widely studied concept in theoretical research. However, if the newly unveiled laws of nature are to be useful, we need to write the dictionary that allows us to translate abstract statements of theoretical quantum thermodynamics to physical platforms and working mediums of experimentally realistic scenarios. To assist in this endeavor, this review is dedicated to providing an overview over the proposed and realized quantum thermodynamic devices, and to highlight the commonalities and differences of the various physical situations.

==> sections/experiment.tex <==
\section{Experimental platforms}

\bla 

==> sections/experiment_QED.tex <==
\subsection{Cavity quantum electrodynamics}

\textbf{\color{red}OBINNA}

\bla 


==> sections/experiment_polariton.tex <==
\subsection{Polariton}

\textbf{\color{red} SEBASTIAN}

\bla 


